Project-based Learning within a Large-Scale Interdisciplinary Research Effort

The modern engineering landscape increasingly requires a range of skills to successfully integrate complex systems. Project-based learning is used to help students build professional skills. However, it is typically applied to small teams and small efforts. This paper describes an experience in engaging a large number of students in research projects within a multi-year interdisciplinary research effort. The projects expose the students to various disciplines in Computer Science (embedded systems, algorithm design, networking), Electrical Engineering (circuit design, wireless communications, hardware prototyping), and Applied Physics (thin-film battery design, solar cell fabrication). While a student project is usually focused on one discipline area, it requires interaction with at least two other areas. Over 5 years, 180 semester-long projects have been completed. The students were a diverse group of high school, undergraduate, and M.S. Computer Science, Computer Engineering, and Electrical Engineering students. Some of the approaches that were taken to facilitate student learning are real-world system development constraints, regular cross-group meetings, and extensive involvement of Ph.D. students in student mentorship and knowledge transfer. To assess the approaches, a survey was conducted among the participating students. The results demonstrate the effectiveness of the approaches. For example, 70% of the students surveyed indicated that working on their research project improved their ability to function on multidisciplinary teams more than coursework, internships, or any other activity.

==> tex/bios.tex <==

\begin{IEEEbiography}{Michael Shell}
Biography text here.
\end{IEEEbiography}

==> tex/lessons_learned.tex <==

Throughout the \mbox{5-year} course of the project, many important lessons were learned.
%Our experiences highlight and reinforce the need to foster opportunities for 

%% From John's version ->
%\subsection{Lessons Learned in Response to Feedback from Undergraduate and M.S. Students}
\par \noindent \textbf{Formalized knowledge transfer process}: A large-scale, long-term project necessitates knowledge transfer between the students. The project used an internal wiki and an external website that were  kept up to date with shared technical information and documentation. While knowledge transfer needs to be carefully monitored and emphasized, most students embraced it when they could see first-hand that the documentation they created was used by their peers and mentors. Similarly, most students embraced the opportunity to introduce peers to their work and to teach them.

\par \noindent \textbf{Well-defined interfaces between student projects}: Some of the most challenging problems arose when a student interfaced his or her project with another project. The difficulty of solving these interface problems in certain cases led to interpersonal tensions. Designing the interfaces between different technologies has been a challenging task that often required faculty members' involvement. Ultimately these issues can only be addressed by establishing, maintaining, and nurturing the connections between the groups and between the different students.

%\subsection{Project Lessons Learned}

\par \noindent\textbf{Risk management:}  The frequent demonstrations of the EnHANTs system necessitated rigorous project management of the many subsystems. The weekly meetings were used to ensure that components were on track for upcoming deadlines, and to adjust the goals accordingly. Off-site demonstrations entailed rigourous contingency planning. Of the many logistics to be considered were international shipping of our testbed, prototypes, and monitoring system and voltage and plug adapters to accommodate international power supplies. Additionally, we prepared 2-3 backup components for each subsystem, extensively testing each of the them while integrated with the rest of the system.

\par \noindent \textbf{Ph.D.\ student development:} Handling many of the day-to-day activities, the Ph.D.\ students quickly learn from their P.I.\ to become advisors to the high school, undergraduate, and M.S. students. This awards them opportunities to practice teaching, assigning deadlines, and motivating their advisees. %, assigning grades.
Additionally, the Ph.D.\ students served as an initial review for all presentation materials, allowing them to practice giving technical and writing feedback. This experience provides the Ph.D.\ students insight into the managerial aspects of future academic positions. These are important high level skills which are also applicable to positions in industry.
%learn to write demonstration abstracts and review presentation materials. learn preparation. different management techniques (visual learners, analytical). almost like teaching experience. young phd students learn from older students. \textbf{THIS TO BE WRITTEN STILL}


\par \noindent \textbf{Real world work environment:}
The experience provided by the EnHANTs project closely resembled industry or graduate school working environments. Students typically join the project at the beginning of the semester and are required to get up to speed in relatively short time frames, similar to Industry jobs. The frequent cross-group meetings and collaboration is akin to many engineering environments.



%% inter-disciplinary work
    %% -- Need for collaborative tools. Need for frequent collaboration.
            %% Encourage students to collaborate at all times
    %% -- Respect for each other -- may be difficult to establish rapport
            %% To establish it, we do things like lunches
    %% -- Practical issues:
            %% Difficult to define interfaces and very difficult to solve technical problems
            %%  without people blaming each others
            %% Gaps in technical skills

%% -- Large-scale: -> Need to showcase individual contributions


\noindent \textbf{Close and continuous cross-group interactions: }The students work in different labs, focus on different disciplines, and have different technical skills, priorities, work styles, and expectations. Early on we discovered that \emph{the gaps between the knowledge of the students with different expertise areas are much wider than anticipated}. For example, Electrical Engineering students
are oftentimes
unfamiliar with good software development practices,
while many Computer Science students may not understand how to properly handle experimental electronics. Additionally, many students that are not majoring in Electrical Engineering do not understand the concepts of frequency-domain signal processing that are essential to the understanding of wireless networking.
These knowledge gaps often lead to both technological and interpersonal issues. Cross-group problem solving requires students to trust each other's expertise, but these gaps in knowledge can make the trust difficult to establish. When working with students we highlight that such gaps are normal and should be treated as a learning opportunity. Ultimately these issues can only be addressed by % \item
\emph{establishing, maintaining, and nurturing the connections between the groups and between the different students}.
%Specifically, we have learned the importance of the following:


%\begin{myitemize}
%%\item
%%\emph{Extensive use of collaborative tools}: As the project has progressed, we have expanded our use of collaborative tools.
%%    The EnHANTs project has an internal wiki and an external website that are
%%    kept up to date with shared technical information and documentation. We use less formal Google docs to keep the students ``on the same page'' with regards to project timelines and tasks.
%
%\item \emph{Well-defined interfaces between student projects}: Some of the most challenging problems arise when a student interfaces his or her project with another project. The difficulty of solving these interface problems can in certain cases lead to interpersonal tensions. Designing the interfaces between different technologies (e.g., solar cells and the energy harvesting module, \mbox{UWB-IR} communication module and the control module) has been a challenging task that often required faculty members' involvement.
%
%%\item \emph{Formalized knowledge transfer process}: A large-scale, long-term project necessitates knowledge transfer between the students. In our experience, while knowledge transfer needs to be carefully monitored and emphasized,
%%    most students embrace it when
%%    they see first-hand that the documentation they create
%%    is
%%    used by their peers. Similarly, most students embrace
%%    the opportunity to introduce peers to their work and to teach them.
%
%%\item \emph{Showcase of individual student contributions}:
%%With many student projects integrated into the prototypes, the contributions of some students may not be as visible as the contributions of others. To address this, we conduct workshops where the students present their projects individually. We also separately showcase each student project on the EnHANTs project website.
%\end{myitemize}



==> tex/recommendations.tex <==


// \textbf{ (Recommendations go here!)}  //


Lessons learned: 

\smallskip 
\noindent \textbf{Importance of knowledge transfer}:

==> tex/students.tex <==

\begin{figure}[t]
\centering
%\hspace{.1in}
\subfigure[\label{fig:studentsAcademLevel}Projects completed in different semesters by students on different levels.]
{\includegraphics[width=0.9\columnwidth]{figs/figsStudents/overTimeByLevel.eps}}
\subfigure[\label{fig:studentsVarious} Student population break-down: by academic level (left) and by project area (middle), and percentage of local students and visitors (right).
]
{
\includegraphics[width=0.485\columnwidth]{figs/figsStudents/academicLevel.eps}
%\hspace{.1in}
\includegraphics[width=0.485\columnwidth]{figs/figsStudents/labs.eps}
%\hspace{.1in}
%\includegraphics[width=0.3\columnwidth]{figs/figsStudents/visitors.eps}
}
%
%\subfigure[By academic level.
%\label{fig:studentsAcademLevel}]{\includegraphics[width=0.35\columnwidth]{figs/figsStudents/academicLevel.eps}}
%\hspace{.1in}
%\subfigure[By research group affiliation. \label{fig:studentsLabs}]{\includegraphics[width=0.35\columnwidth]{figs/figsStudents/labs.eps}}
%\hspace{.1in}
%\subfigure[University students vs.\ visitors.
%\label{fig:studentsVisitors}]{\includegraphics[width=0.35\columnwidth]{figs/figsStudents/visitors.eps}}
%\subfigure[By gender.
%\label{fig:studentsGender}]{\includegraphics[width=0.45\columnwidth]{figs/figsStudents/gender.eps}}
%\subfigure[Academic outcome, out of total 29 graduated students (continuing students not included).
%\label{fig:studentsOutcome}]{\includegraphics[width=0.45\columnwidth]{figs/figsStudents/outcome.eps}}
%\hspace{.1in}
%\subfigure[\label{fig:overTimePhase}]{\includegraphics[width=0.8\columnwidth]{figs/figsStudents/overTimeByPhase.eps}}
%\hspace{.1in}
\vspace*{-0.25cm}
\caption{Participating students: (a) percentage breakdown of the total number of students involved by different parameters (51 students total), and (b) projects completed in different semesters, by students at different academic levels. %The total number of students: 51. Percentage breakdowns in various ways are demonstrated.
\label{fig:studentBreakdown}}
\end{figure}


%\smallskip
%\par \noindent
%\textbf{Students at different levels working together}: at any given point, students at various academic %levels worked together.

The participating students were a highly diverse group, as shown in Fig.~\ref{fig:studentBreakdown}. %demonstrates graphically several student breakdowns.
Out of 51 students involved in the work, 6\% were high school students, 31\% -- undergraduates, 50\% - M.S.\ students, and the remaining 13\% were Ph.D.\ students (Fig.~\ref{fig:studentsVarious}). %similar percentages of projects completed by students at different levels throughout different semesters (Fig.~\ref{fig:studentsAcademLevel}).
Student projects' main focus was networking (50\%), wireless communications (25\%), electronics (15\%), and distributed systems, operating systems, and others (10\% in total).
% While 75\% of students were enrolled in programs in the home university, 25\% of students were visiting students and researchers from different universities, closely located, as well as international.




\iffalse 
\begin{figure}[t]
\centering
\subfigure[]{
\includegraphics[width=0.6\columnwidth]{figs/figsStudents/academicLevel.eps}}
\subfigure[]{\includegraphics[width=0.6\columnwidth]{figs/figsStudents/labs.eps}}
\vspace*{-0.25cm}
\caption{\label{fig:studentsVarious} Student population break-down: (a) by academic level, and (b) by project area. \label{fig:studentBreakdown}}
\end{figure}
\fi




\iffalse
%%%% Students over time
\begin{figure}[t]
\centering
%\subfigure[\label{fig:overTimeLevel}]
%{
\includegraphics[width=0.9\columnwidth]{figs/figsStudents/overTimeByLevel.eps}
%}
\vspace*{-0.25cm}
\caption{Student projects completed in different semesters, by student level. \label{fig:studentsOverTime}}
\end{figure}
\fi



\iffalse
%%%% Students over time
\begin{figure}[t]
\centering
\subfigure[\label{fig:overTimePhase}]{\includegraphics[width=0.8\columnwidth]{figs/figsStudents/overTimeByPhase.eps}}
\vspace*{-0.25cm}
\caption{[]\label{fig:studentsOverTime}}
\end{figure}
\fi

%Student contributions by projects


\iffalse
Of the projects done by undergraduate and Masters students, 64 (ZZ\%) were `core' testbed projects that required interactions between many different labs.  %%On average, 10.45 student project per semester have been completed.
\fi

%been directly involved in this project.\footnote{We only count students and the semesters that were involved in the project for more than 2 hours per week. We do not include students that, for example, provided software support, but did not participate in the project.} Out of the 51, 3 were high school students, 16 -- undergraduate, 26 --- Masters, and 6 were PhD students. 38 students were Columbia University-affiliated, while 13 were visitors, from other local schools or universities, as well as visitors from abroad.

%Many students have dedicated more than one semester to the project.
\iffalse Altogether, students have completed 115 semester-long projects (`student-semesters'); the majority of student projects (107, 93\%) were completed by students involved in the following three labs: networking (Wim.Net), materials (CLUE), and electronics (CISL) labs.\footnote{The remaining 8 student semester projects were completed within distributed computing and wireless communications labs.}
\fi

%% do: display by student types
%For example, between the two phases shown in

%
%\begin{itemize}
%\item Count: students who directly worked on interfacing ``CS'' with ``non-CS'' (or on a disciplinary boundary in general)
%\item Count: students by graduate student superviser
%\end{itemize}


